Counterfactual Explanations Using Optimization With Constraint Learning

To increase the adoption of counterfactual explanations in practice, several criteria that these should adhere to have been put forward in the literature. We propose counterfactual explanations using optimization with constraint learning (CE-OCL), a generic and flexible approach that addresses all these criteria and allows room for further extensions. Specifically, we discuss how we can leverage an optimization with constraint learning framework for the generation of counterfactual explanations, and how components of this framework readily map to the criteria. We also propose two novel modeling approaches to address data manifold closeness and diversity, which are two key criteria for practical counterfactual explanations. We test CE-OCL on several datasets and present our results in a case study. Compared against the current state-of-the-art methods, CE-OCL allows for more flexibility and has an overall superior performance in terms of several evaluation metrics proposed in related work.

==> CE-OCL arXiv 2/sibcommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                             %
%  Prepared by S. Ilker Birbil.       Date: February, 2019    %
%                                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Auxiliary Commands
% \setuptodonotes{backgroundcolor=red!10, linecolor=red,
%   bordercolor=red, size=\tiny, shadow, tickmarkheight=0.1cm}

% \newcommand\hlb[3][]{\todo[inline,caption={emptytext},
%   size=\normalsize, backgroundcolor=yellow!70, bordercolor=yellow!70, noshadow, #1]{
%     \begin{minipage}{
%         \textwidth-4pt}#2
%     \end{minipage}}
%   \todo{\begin{spacing}{0.5}#3\end{spacing}}}

% \newcommand{\hlc}[2]{\hl{#1}\todo{\begin{spacing}{0.5}#2\end{spacing}}}

% \newcommand{\sitodo}[2][]{\todo[caption={#2}, #1]{
%     \begin{spacing}{0.5}#2\end{spacing}}}

% \newcommand{\intodo}[2][]{\todo[inline, noshadow, caption={emptytext}, #1]{
%    \begin{spacing}{1.0}\normalsize{#2}\end{spacing}}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\magenta}[1]{\textcolor{magenta}{#1}}
\newcommand{\sibm}[1]{\mbox{\boldmath{$#1$}}}
\newcommand{\rb}[1]{\raisebox{-1.5ex}[0cm][0cm]{#1}}
\newcommand{\HRule}{\noindent\rule{\linewidth}{0.5mm}}
\newcommand{\dsum}{\displaystyle\sum}
\newcommand{\veps}{\varepsilon}

\newcommand{\CA}{\mathcal{A}}
\newcommand{\CB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\CD}{\mathcal{D}}
\newcommand{\CG}{\mathcal{G}}
\newcommand{\CI}{\mathcal{I}}
\newcommand{\CJ}{\mathcal{J}}
\newcommand{\CK}{\mathcal{K}}
\newcommand{\CL}{\mathcal{L}}
\newcommand{\CN}{\mathcal{N}}
\newcommand{\CP}{\mathcal{P}}
\newcommand{\CS}{\mathcal{S}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\CX}{\mathcal{X}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}

\newcommand{\va}{\sibm{a}}
\newcommand{\vb}{\sibm{b}}
\newcommand{\vc}{\sibm{c}}
\newcommand{\vd}{\sibm{d}}
\newcommand{\ve}{\sibm{e}}
\newcommand{\vf}{\sibm{f}}
\newcommand{\vg}{\sibm{g}}
\newcommand{\vp}{\sibm{p}}
\newcommand{\vr}{\sibm{r}}
\newcommand{\vs}{\sibm{s}}
\newcommand{\vt}{\sibm{t}}
\newcommand{\vu}{\sibm{u}}
\newcommand{\vv}{\sibm{v}}
\newcommand{\vw}{\sibm{w}}
\newcommand{\vx}{\sibm{x}}
\newcommand{\vy}{\sibm{y}}
\newcommand{\vz}{\sibm{z}}
\newcommand{\zv}{\sibm{0}}
\newcommand{\ov}{\sibm{1}}

\newcommand{\veta}{\sibm{\eta}}
\newcommand{\vxi}{\sibm{\xi}}
\newcommand{\valpha}{\sibm{\alpha}}
\newcommand{\vbeta}{\sibm{\beta}}
\newcommand{\vgamma}{\sibm{\gamma}}
\newcommand{\vtheta}{\sibm{\theta}}
\newcommand{\vlambda}{\sibm{\lambda}}
\newcommand{\vnu}{\sibm{\nu}}
\newcommand{\vmu}{\sibm{\mu}}
\newcommand{\vdelta}{\sibm{\delta}}

\newcommand{\mA}{\sibm{A}}
\newcommand{\mB}{\sibm{B}}
\newcommand{\mC}{\sibm{C}}
\newcommand{\mD}{\sibm{D}}
\newcommand{\mE}{\sibm{E}}
\newcommand{\mF}{\sibm{F}}
\newcommand{\mG}{\sibm{G}}
\newcommand{\mH}{\sibm{H}}
\newcommand{\mI}{\sibm{I}}
\newcommand{\mL}{\sibm{L}}
\newcommand{\mM}{\sibm{M}}
\newcommand{\mP}{\sibm{P}}
\newcommand{\mQ}{\sibm{Q}}
\newcommand{\mR}{\sibm{R}}
\newcommand{\mS}{\sibm{S}}
\newcommand{\mU}{\sibm{U}}
\newcommand{\mV}{\sibm{V}}
\newcommand{\mX}{\sibm{X}}

\newcommand{\tr}{^{\intercal}}
\newcommand{\ntr}{^{-\intercal}}
\newcommand{\inv}{^{-1}}

\newcommand{\gr}{\mbox{graph}}
\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\rra}{\rightrightarrows}
\newcommand{\ptr}{\marginpar{$\Leftarrow$}}

\newcommand{\pfxi}{\frac{\partial f(\vx)}{\partial x_i}}
\newcommand{\pfx}{\partial f(\vx)}
\newcommand{\pf}{\partial f}
\newcommand{\pxi}{\partial x_i}
\newcommand{\px}{\partial x}

\newcommand{\nfx}{\nabla f(\vx)}
\newcommand{\eps}{\epsilon}
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\ie}{\textit{i.e.}}

\newcommand{\vsp}{\vspace{4mm}}
\newcommand{\vspp}{\vspace{8mm}}
\newcommand{\vsppp}{\vspace{12mm}}

\newcommand{\hsp}{\hspace{4mm}}
\newcommand{\hspp}{\hspace{8mm}}
\newcommand{\hsppp}{\hspace{12mm}}

\newcommand{\pr}[1]{\mathbb{P}\left\{#1\right\}}
\newcommand{\ex}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\variance}[1]{\mbox{Var}\left(#1\right)}
\newcommand{\covar}[1]{\mbox{Cov}\left(#1\right)}
\newcommand{\C}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}

\newcommand{\maximize}{\mbox{maximize\hspace{4mm} }}
\newcommand{\minimize}{\mbox{minimize\hspace{4mm} }}
\newcommand{\subto}{\mbox{subject to\hspace{4mm}}}

\newenvironment{SIBitemize}{
  \renewcommand{\labelitemi}{$\diamond$}
  \begin{itemize}
    \setlength{\parskip}{0mm}}
  {\end{itemize}}

% \newcounter{commentcounter}
% \setcounter{commentcounter}{1}

% \newcommand{\commentin}[1]{\newline\fbox{\parbox{15cm}{
%       \noindent\footnotesize{\texttt{
%           \textcolor{red}{(C.\arabic{commentcounter})~#1}}}}}
%   \newline \addtocounter{commentcounter}{1} }

% \long\def\symbolfootnote[#1]#2{\begingroup
%   \def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
% \newcommand{\comment}[1]{{\footnotesize\textbf{
%       \textcolor{red}{(C.\arabic{commentcounter})}}
%     \symbolfootnote[4]{\texttt{\textcolor{red}
%         {(C.\arabic{commentcounter})~ #1}}}}
%   \addtocounter{commentcounter}{1}}

% \newcommand{\commentside}[1]{{\footnotesize\textbf{
%       \textcolor{red}{(C.\arabic{commentcounter})}}}
%   \mbox{}\marginpar[\raggedleft\hspace{0pt}\footnotesize{\texttt{
%       \textcolor{red}{(C.\arabic{commentcounter})$\blacktriangleright$\\
%         \parbox{1.5cm}{#1}}}}]{\raggedright\hspace{0pt}\footnotesize{
%       \texttt{\textcolor{red}{$\blacktriangleleft$(C.\arabic{commentcounter})\\
%           \parbox{1.5cm}{#1}}}}}\addtocounter{commentcounter}{1}}

\newcommand{\propnum}[2]{\vspace{3mm}
  \noindent {\sc Proposition #1}{\it #2} \vspace{3mm}}
\newcommand{\lemnum}[2]{\vspace{3mm}
  \noindent {\sc Lemma #1}{\it #2} \vspace{3mm}}
\newcommand{\thmnum}[2]{\vspace{3mm}
  \noindent {\sc Theorem #1}{\it #2} \vspace{3mm}}
\newcommand{\intodo}[2][]{\todo[inline, noshadow, caption={emptytext}, #1]{
    \begin{spacing}{1.0}\normalsize{#2}\end{spacing}}}
    

==> CE-OCL arXiv 2/tables/dice_comparison_w_compas.tex <==
\renewcommand{\baselinestretch}{0.95} 

\begin{table}[ht]
    \caption{Comparison of CE-OCL, CE-OCL with trust region, and DiCE (genetic) with a range of preditive models.}
    
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}

\resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lllllllll@{}}
\begin{tabular}{p{0.5cm}p{2cm}p{1.8cm}p{2cm}p{3.7cm}p{2cm}p{2cm}p{3.5cm}p{2.5cm}}
% \begin{tabular}{p{0.8cm}p{1.8cm}p{2.3cm}p{2.3cm}r{3cm}p{2cm}p{2.3cm}r{3.7cm}p{2cm}}
% \begin{tabular}{@{}llccccccc@{}}
\toprule
        & & \textbf{validity}($\uparrow_0^1$)  &  \textbf{cat. pro-} &  \textbf{cont.} &  \textbf{sparsity}($\uparrow_0^1$) &  \textbf{cat. di-} &  \textbf{cont.} &  \textbf{sparsity-based} \\ [-1mm]
        & &   & \textbf{ximity} ($\uparrow_0^1$)  &  \textbf{proximity}($\uparrow_-^0$)&  & \textbf{versity} ($\uparrow_0^1$) & \textbf{diversity} ($\uparrow_0^+$) &  \textbf{diversity}($\uparrow_0^1$) \\ 
        & & mean (s.e.) & mean (s.e.) & mean (s.e.) & mean (s.e.) & mean (s.e.)  & mean (s.e.) & mean (s.e.) \\ \midrule
\multicolumn{9}{c}{\textbf{Adult dataset}}\\ \midrule
\rowcolor{gray!10}                                      & CE-OCL        & \textbf{1.00} (0.00) & \textbf{0.99} (0.00) & \textbf{-6775.61} (953.24)     & \textbf{0.92} (0.00) & 0.01 (0.01) & 5796.61 (1056.70)    & 0.11 (0.01)        \\
\rowcolor{gray!10} rf                                          & CE-OCL\_tr    & \textbf{1.00} (0.00) & 0.97 (0.02) & -25044.04 (7645.82)   & 0.86 (0.01) & 0.00 (0.00) & 13288.83 (3236.28)   & 0.13 (0.01)        \\
\rowcolor{gray!10}                                          & DiCE & 1.00 (0.00) & 0.74 (0.02) & -81581.97 (8003.12)   & 0.51 (0.01) & \textbf{0.19} (0.02) & \textbf{79595.54} (7496.70)   & \textbf{0.26} (0.02)        \\ 

% \midrule

                                        & CE-OCL        & \textbf{1.00} (0.00) & \textbf{0.99} (0.01) & \textbf{-4226.05} (794.33)     & \textbf{0.89} (0.01) & 0.01 (0.01) & 8042.59 (1418.66)    & 0.19 (0.01)        \\
lr                                          & CE-OCL\_tr    & \textbf{1.00} (0.00) & 0.96 (0.02) & -23288.53 (6837.94)   & 0.84 (0.01) & 0.05 (0.02) & 23421.06 (7376.79)   & 0.22 (0.01)        \\
                                          & DiCE & 0.71 (0.05) & 0.68 (0.03) & -111661.60 (10261.28) & 0.47 (0.02) & \textbf{0.30} (0.03) & \textbf{110668.36} (11019.56) & \textbf{0.35} (0.02)        \\ 
                                          
                                        %   \midrule
                                          
\rowcolor{gray!10}                                        & CE-OCL        & \textbf{1.00} (0.00) & 0.88 (0.02) & \textbf{-13994.62} (4198.07)   & 0.83 (0.02) & 0.21 (0.04) & 26889.72 (8343.13)   & \textbf{0.27} (0.03)        \\
\rowcolor{gray!10} cart                                      & CE-OCL\_tr    & \textbf{1.00} (0.00) & \textbf{0.94} (0.01) & -19490.98 (5725.22)   & \textbf{0.84} (0.01) & 0.08 (0.02) & 20313.32 (5702.44)   & 0.19 (0.01)        \\
\rowcolor{gray!10}                                           & DiCE  & 0.65 (0.06) & 0.77 (0.02) & -91507.16 (10271.17)  & 0.55 (0.02) & \textbf{0.23} (0.02) & \textbf{84111.77} (11802.96)  & 0.25 (0.01)        \\ 

% \midrule

                                          & CE-OCL        & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & \textbf{-10553.10} (1842.00)   & \textbf{0.88} (0.01) & 0.00 (0.00) & 2538.19 (669.37)     & 0.15 (0.02)        \\
mlp                                          & CE-OCL\_tr    & \textbf{1.00} (0.00) & 0.97 (0.02) & -21467.01 (7465.77)   & 0.86 (0.01) & 0.00 (0.00) & 6229.99 (2385.40)    & 0.14 (0.01)        \\
                                          & DiCE & 0.62 (0.06) & 0.67 (0.03) & -89314.87 (10646.04)  & 0.47 (0.02) & \textbf{0.26} (0.03) & \textbf{83848.59} (11476.56)  & \textbf{0.31} (0.02)        
                                          \\ 
                                        %   \midrule
                                          
\rowcolor{gray!10}                                          & CE-OCL        & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & \textbf{-2488.82} (865.72)     & \textbf{0.91} (0.00) & 0.00 (0.00) & 4475.59 (1737.16)    & 0.13 (0.01)        \\
\rowcolor{gray!10} gbm                                          & CE-OCL\_tr    & \textbf{1.00} (0.00) & 0.97 (0.01) & -22732.34 (7545.41)   & 0.88 (0.01) & 0.02 (0.01) & 10609.72 (3583.71)   & 0.15 (0.01)        \\
\rowcolor{gray!10}                                          & DiCE & 0.91 (0.04) & 0.70 (0.02) & -113297.47 (11606.39) & 0.49 (0.01) & \textbf{0.25} (0.02) & \textbf{75728.74} (10042.23)  & \textbf{0.27} (0.02)        \\ \bottomrule
\end{tabular}%
}

\resizebox{\textwidth}{!}{%
% \begin{tabular}{p{0.5cm}p{2cm}p{2.5cm}p{3cm}p{3.2cm}p{2.5cm}p{2.5cm}p{3cm}p{2.5cm}}
\begin{tabular}{p{0.5cm}p{2cm}p{1.8cm}p{2cm}p{3.7cm}p{2cm}p{2cm}p{3.5cm}p{2.5cm}}
% \begin{tabular}{@{}lllllllll@{}}
\multicolumn{9}{c}{\textbf{COMPAS dataset}}\\ \midrule

\rowcolor{gray!10}                     & CE-OCL     & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & \textbf{-18.79} (6.15)   & \textbf{0.85} (0.00) & 0.00 (0.00) & 8.87 (4.30)    & 0.17 (0.01) \\
\rowcolor{gray!10} rf                   & CE-OCL\_tr & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & -38.02 (16.46)  & \textbf{0.85} (0.01) & 0.00 (0.00) & 9.41 (4.49)    & 0.16 (0.01) \\
\rowcolor{gray!10}                     & DiCE       & 0.81 (0.04) & 0.96 (0.01) & -40.94 (7.06)   & 0.60 (0.01) & \textbf{0.06} (0.02) & \textbf{22.30} (5.78)   & \textbf{0.20} (0.01) \\ 

% \midrule

                     & CE-OCL     & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & -121.74 (13.72) & \textbf{0.80} (0.01) & 0.00 (0.00) & \textbf{229.89} (28.27) & 0.34 (0.01) \\
lr               & CE-OCL\_tr & \textbf{1.00} (0.00) & 0.98 (0.01) & \textbf{-35.84} (11.03)  & 0.75 (0.01) & 0.01 (0.01) & 34.68 (7.79)   & \textbf{0.35} (0.01) \\
                     & DiCE       & 0.85 (0.05) & 0.94 (0.02) & -56.05 (12.83)  & 0.59 (0.01) & \textbf{0.08} (0.02) & 30.61 (9.48)   & 0.21 (0.02) \\ 
                     
                    %  \midrule
                     
\rowcolor{gray!10}                     & CE-OCL     & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & \textbf{-23.14} (6.03)   & \textbf{0.84} (0.01) & 0.00 (0.00) & \textbf{33.38} (11.83)  & \textbf{0.19} (0.01) \\
\rowcolor{gray!10} cart                 & CE-OCL\_tr & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & -28.43 (9.16)   & 0.83 (0.01) & 0.00 (0.00) & 31.16 (10.10)  & \textbf{0.19} (0.01) \\
\rowcolor{gray!10}                     & DiCE       & 0.77 (0.08) & 0.96 (0.01) & -32.99 (6.04)   & 0.60 (0.01) & \textbf{0.07} (0.02) & 24.31 (6.63)   & 0.18 (0.01) \\ 

% \midrule

                     & CE-OCL     & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & \textbf{-16.55} (2.11)   & 0.81 (0.01) & 0.00 (0.00) & 16.20 (4.62)   & \textbf{0.22} (0.01) \\
mlp                  & CE-OCL\_tr & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & -27.75 (10.25)  & \textbf{0.82} (0.01) & 0.00 (0.00) & 7.29 (4.09)    & 0.18 (0.01) \\
                     & DiCE       & 0.82 (0.06) & 0.96 (0.01) & -59.11 (13.01)  & 0.58 (0.01) & \textbf{0.06} (0.02) & \textbf{24.95} (5.78)   & \textbf{0.22} (0.02) \\ 
                     
                    %  \midrule
                     
\rowcolor{gray!10}                     & CE-OCL     & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & \textbf{-10.10} (2.60)   & \textbf{0.86} (0.00) & 0.00 (0.00) & 13.64 (3.09)   & \textbf{0.21} (0.01) \\
\rowcolor{gray!10} gbm                  & CE-OCL\_tr & \textbf{1.00} (0.00) & \textbf{1.00} (0.00) & -25.70 (10.66)  & 0.85 (0.01) & 0.00 (0.00) & 13.49 (5.08)   & 0.20 (0.01) \\
\rowcolor{gray!10}                     & DiCE       & 0.59 (0.07) & 0.96 (0.01) & -42.64 (6.32)   & 0.60 (0.01) & \textbf{0.08} (0.02) & \textbf{24.51} (5.81)   & 0.20 (0.01) \\ 
\bottomrule
\end{tabular}%
}


% \begin{longtable}{@{}lllllllll@{}}

\resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lllllllll@{}}
% \begin{tabular}{p{0.5cm}p{2cm}p{2.5cm}p{3cm}p{3.2cm}p{2.5cm}p{2.5cm}p{3cm}p{2.5cm}}
\begin{tabular}{p{0.5cm}p{2cm}p{1.8cm}p{2cm}p{3.7cm}p{2cm}p{2cm}p{3.5cm}p{2.5cm}}
\multicolumn{9}{c}{\textbf{Heloc dataset}}\\ \midrule

\rowcolor{gray!10}                     & CE-OCL     & \textbf{1.00} (0.00) & -- & \textbf{-13.53} (2.35)   & \textbf{0.93} (0.00) & -- & 9.94 (2.74)    & 0.09 (0.01) \\
\rowcolor{gray!10} rf                   & CE-OCL\_tr & \textbf{1.00} (0.00) & -- & -94.24 (13.68)  & 0.75 (0.02) & -- & 18.93 (4.62)   & 0.24 (0.02) \\
\rowcolor{gray!10}                     & DiCE       & 0.90 (0.03) & -- & -231.05 (11.17) & 0.21 (0.02) & -- & \textbf{223.91} (14.16) & \textbf{0.61} (0.02) \\ 
                     
                    %  \midrule
                     
                     
                     & CE-OCL     & \textbf{1.00} (0.00) & -- & \textbf{-99.09} (14.22)  & \textbf{0.88} (0.01) & -- & 188.16 (28.38) & 0.21 (0.01) \\
lr               & CE-OCL\_tr & \textbf{1.00} (0.00) & -- & -138.29 (16.52) & 0.72 (0.02) & -- & 72.51 (8.39)   & 0.34 (0.02) \\
                     & DiCE       & 0.70 (0.06) & -- & -232.39 (12.87) & 0.21 (0.02) & -- & \textbf{207.02} (11.34) & \textbf{0.61} (0.02) \\ 
                     
                    %  \midrule
                     
\rowcolor{gray!10}                     & CE-OCL     & \textbf{1.00} (0.00) & -- & \textbf{-13.12} (1.40)   & \textbf{0.95} (0.00) & -- & 19.72 (2.41)   & 0.08 (0.00) \\
\rowcolor{gray!10} cart                 & CE-OCL\_tr & \textbf{1.00} (0.00) & -- & -99.05 (13.45)  & 0.73 (0.02) & -- & 41.03 (6.53)   & 0.31 (0.02) \\
\rowcolor{gray!10}                     & DiCE       & 0.80 (0.07) & -- & -216.70 (13.47) & 0.22 (0.02) & -- & \textbf{234.89} (16.10) & \textbf{0.61} (0.02) \\ 
                     
                    %  \midrule
                     
                     & CE-OCL     & \textbf{1.00} (0.00) & -- & \textbf{-25.09} (7.57)   & \textbf{0.92} (0.01) & -- & 21.30 (4.18)   & 0.12 (0.01) \\
mlp                  & CE-OCL\_tr & \textbf{1.00} (0.00) & -- & -98.94 (15.87)  & 0.75 (0.02) & -- & 15.41 (5.52)   & 0.26 (0.02) \\
                     & DiCE       & 0.67 (0.07) & -- & -252.56 (14.17) & 0.20 (0.02) & -- & \textbf{246.96} (16.31) & \textbf{0.61} (0.02) \\ 
                     
                    %  \midrule
                     
\rowcolor{gray!10}                     & CE-OCL     & \textbf{1.00} (0.00) & -- & \textbf{-8.41} (2.45)    & \textbf{0.94} (0.00) & -- & 16.31 (4.92)   & 0.10 (0.00) \\
\rowcolor{gray!10} gbm                  & CE-OCL\_tr & \textbf{1.00} (0.00) & -- & -89.91 (14.70)  & 0.76 (0.02) & -- & 18.70 (6.87)   & 0.25 (0.02) \\
\rowcolor{gray!10}                     & DiCE       & 0.73 (0.08) & -- & -234.96 (11.60) & 0.22 (0.02) & -- & \textbf{248.95} (17.34) & \textbf{0.59} (0.02) \\


\bottomrule
\end{tabular}%
}

% \begin{longtable}{@{}lllllllll@{}}

\resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lllllllll@{}}
% \begin{tabular}{p{0.5cm}p{2cm}p{2.5cm}p{3cm}p{3.2cm}p{2.5cm}p{2.5cm}p{3cm}p{2.5cm}}
\begin{tabular}{p{0.5cm}p{2cm}p{1.8cm}p{2cm}p{3.7cm}p{2cm}p{2cm}p{3.5cm}p{2.5cm}}
\multicolumn{9}{c}{\textbf{Give me some credit dataset}}\\ \midrule

\rowcolor{gray!10}                    & CE-OCL     & \textbf{1.00} (0.00) & -- & \textbf{-6.77} (4.43)      & \textbf{0.90} (0.00) & -- & 9.14 (5.53)      & 0.15 (0.01) \\
\rowcolor{gray!10} rf                   & CE-OCL\_tr & \textbf{1.00} (0.00) & -- & -97.01 (95.21)    & 0.89 (0.01) & -- & 115.65 (113.90)  & 0.16 (0.01) \\
\rowcolor{gray!10}                     & DiCE       & \textbf{1.00} (0.00) & -- & -2166.72 (318.36) & 0.23 (0.02) & -- & \textbf{2446.71} (455.17) & \textbf{0.32} (0.01) \\
                     
                    %  \midrule
                     
                     & CE-OCL     & \textbf{1.00} (0.00) & -- & \textbf{-3.79} (1.24)      & \textbf{0.88} (0.01) & -- & 7.50 (2.49)      & 0.24 (0.01) \\
lr               & CE-OCL\_tr & \textbf{1.00} (0.00) & -- &   -614.00 (202.97)           &     0.83 (0.01)        & -- & 1107.84 (381.92)                  &  0.25 (0.01)           \\
                     & DiCE       & 0.92 (0.05) & -- & -1946.86 (256.37) & 0.21 (0.02) & -- & \textbf{1909.26} (187.85) & \textbf{0.29} (0.01) \\ 
                     
                    %  \midrule
                     
\rowcolor{gray!10} & CE-OCL     & \textbf{1.00} (0.00) & -- & -1.85 (0.23)      & \textbf{0.87} (0.00) & -- & 1.91 (0.23)      & 0.17 (0.00) \\
\rowcolor{gray!10} cart                 & CE-OCL\_tr & \textbf{1.00} (0.00) & -- &  -212.82 (100.91)                 &  0.85 (0.01)           & -- &     285.60 (121.56)             &       0.22 (0.01)      \\
\rowcolor{gray!10}                     & DiCE       & 0.00 (0.00) & -- & -1895.95 (230.21) & 0.25 (0.02) & -- & \textbf{2214.51} (319.98) & \textbf{0.32} (0.01) \\
                     
                    %  \midrule
                     
                     & CE-OCL     & \textbf{1.00} (0.00) & -- & \textbf{-24.21} (8.71)     & \textbf{0.89} (0.00) & -- & 38.15 (13.75)    & 0.15 (0.01) \\
mlp                  & CE-OCL\_tr & \textbf{1.00} (0.00) & -- & -996.30 (370.04) & 0.85 (0.01)  & -- &  971.37 (447.54)                &  0.17 (0.01)           \\
                     & DiCE       & 0.97 (0.03) & -- & -2526.22 (265.46) & 0.20 (0.02) & -- & \textbf{3205.58} (427.42) & \textbf{0.32} (0.01) \\
                     
                    %  \midrule
                     
\rowcolor{gray!10}                     & CE-OCL     & \textbf{1.00} (0.00) & -- &    \textbf{-175.98} (74.32)               &    \textbf{0.89} (0.01)         & -- &     296.26 (134.93)             &  0.17 (0.01)           \\
\rowcolor{gray!10} gbm                  & CE-OCL\_tr & \textbf{1.00} (0.00) & -- & -219.19 (131.96)           &     0.87 (0.01)        & -- &    123.61 (82.17)              &    0.16 (0.01)          \\
\rowcolor{gray!10}                     & DiCE       &  0.93 (0.04)           & -- &   -2222.50 (277.89)                &   0.22 (0.02)          & -- &    \textbf{2749.12} (409.75)              &     \textbf{0.31} (0.02)        \\


\bottomrule
\end{tabular}%
}







    
    
    \label{tab:ce-ocl_vs_dice}
\end{table}

==> CE-OCL arXiv 2/tables/tab_carla_w_compas.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\renewcommand{\baselinestretch}{1}
\begin{table}[ht]
\caption{Comparison of CE-OCL with DiCE (genetic), Algorithmic Recourse, Growing spheres, and FACE using Random Forest as predictive model.}
\label{tab:carla_comparison}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llcclc@{}}
\toprule
                              &                           & \textbf{validity} ($\uparrow_0^1$)       & \textbf{cat. proximity} ($\uparrow_0^1$)       & \textbf{cont. proximity} ($\uparrow_-^0$)      & \textbf{sparsity} ($\uparrow_0^1$)      \\
                              &                           & mean (s.e.)                     & mean (s.e.)                                  & mean (s.e.)                                & mean (s.e.)       \\ \midrule
\rowcolor{gray!10}                & CE-OCL                       & \textbf{1.00} (0.00)                        & \textbf{1.00} (0.00)                                    & -4844.35 (575.93)                             & \textbf{0.93} (0.00)                       \\
\rowcolor{gray!10} & CE-OCL\_tr & \textbf{1.00} (0.00) & 0.97 (0.02) & -21785.50 (7506.35) & 0.86 (0.01) \\
\rowcolor{gray!10}                & DiCE                & \textbf{1.00} (0.00)                        & 0.74 (0.03)                                    & -84278.61 (11613.30)                          & 0.50 (0.02)                       \\
\rowcolor{gray!10} ADULT           & Actionable Recourse          & \textbf{1.00} (0.00)                        & 0.78 (0.07)                                    & \textbf{0.00} (0.00)                                   & 0.89 (0.04)                       \\
\rowcolor{gray!10}                & Growing Spheres              & 0.80 (0.07)                        & 0.95 (0.01)                                    & -78901.08 (10395.08)                          & 0.59 (0.01)                       \\
\rowcolor{gray!10}                & FACE                         & 0.80 (0.07)                        & 0.65 (0.03)                                    & -108614.33 (18804.05)                         & 0.47 (0.02)                       \\ 
% \midrule
                & CE-OCL                       & \textbf{1.00} (0.00)                        & \textbf{1.00} (0.00)                                    & -15.23 (5.84)                                 & \textbf{0.85} (0.01)                       \\
                & CE-OCL\_tr & \textbf{1.00} (0.00) & 1.00 (0.00) & -30.83 (16.00) & \textbf{0.85} (0.01) \\
                & DiCE                & 0.74 (0.09)                        & 0.94 (0.03)                                    & -35.58 (9.59)                                 & 0.61 (0.01)                       \\
COMPAS          & Actionable Recourse          & 0.67 (0.11)                        & 0.94 (0.03)                                    & \textbf{-0.87} (0.10)                                  & \textbf{0.85} (0.01)                       \\
                & Growing spheres              & 0.80 (0.07)                        & 0.98 (0.02)                                    & -39.88 (6.58)                                 & 0.56 (0.01)                       \\
                & FACE                         & 0.80 (0.07)                        & 0.65 (0.05)                                    & -98.83 (21.18)                                & 0.37 (0.03)                       \\ 
                % \midrule
\rowcolor{gray!10}                & CE-OCL                       & \textbf{1.00} (0.00)                        & --                                             & \textbf{-12.21} (2.67)                                 & \textbf{0.94} (0.01)                       \\
\rowcolor{gray!10} & CE-OCL\_tr & \textbf{1.00} (0.00) & -- & -92.71 (13.75) & 0.75 (0.02) \\
\rowcolor{gray!10}                & DiCE                         & 0.97 (0.03)                        & --                                             & -203.83 (13.70)                               & 0.22 (0.02)                       \\
\rowcolor{gray!10} HELOC           & Actionable Recourse$^*$ & --                                 & --                                             & --                                            & --                                \\
\rowcolor{gray!10}                & Growing spheres              & 0.77 (0.08)                        & --                                             & -87.36 (13.16)                                & 0.00 (0.00)                       \\
\rowcolor{gray!10}                & FACE                         & 0.77 (0.08)                        & --                                             & -361.80 (25.20)                               & 0.17 (0.02)                       \\ 
% \midrule
                & CE-OCL                       & \textbf{1.00} (0.00)                        & --                                             & \textbf{-1.18} (0.66)                                  & \textbf{0.90} (0.01)                       \\
                & CE-OCL\_tr & \textbf{1.00} (0.00) & -- & -120.61 (118.54) & 0.87 (0.01) \\
                & DiCE                         & \textbf{1.00} (0.00)                        & --                                             & -1618.33 (305.53)                             & 0.25 (0.02)                       \\
 CREDIT          & Actionable Recourse          & 0.83 (0.17)                        & --                                             & -8.47 (7.96)                                  & 0.88 (0.02)                       \\
                & Growing spheres              & 0.63 (0.09)                        & --                                             & -47.73 (27.24)                                & 0.10 (0.00)                       \\
                & FACE                         & 0.63 (0.09)                        & --                                             & -3001.73 (430.61)                             & 0.11 (0.02)                       \\
\bottomrule
\multicolumn{6}{l}{\footnotesize For the comparison, one counterfactual was generated for each of 30 factual instances.} \\ [-2mm]
\multicolumn{6}{l}{\footnotesize The scores were averaged over all instances, and the standard error was derived.} \\  [-2mm] 
\multicolumn{6}{l}{\footnotesize * For the Heloc dataset, Actionable Recourse did not yield any counterfactuals for any of the thirty factual instances.} \\
\end{tabular}%
}
\end{table}

==> CE-OCL arXiv 2/tables/table_demo_heart.tex <==
\renewcommand{\baselinestretch}{1.5} 

\begin{table}[h]
\caption{CE-OCL demo on the Statlog (Heart) Data Set \citep[][]{Dua:2019}}
% \begin{subtable}[h]{\textwidth}
\centering
% \caption{Counterfactual explanations generated for enriching the optimization model step by step with the constraint presented in Section~\ref{sec:generate}}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\multicolumn{14}{l}{\LARGE (a) Counterfactual explanations generated for enriching the optimization model step by step with the} \\
\multicolumn{14}{l}{\LARGE constraint presented in Section~\ref{sec:generate}}\\
\toprule
 & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}age} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}bp} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}sch} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}mhrt} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}opk} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}chp} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}ecg} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}exian} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}fbs} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}sex} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}slope} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}thal} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}vessel} \\ \midrule
\rowcolor{gray!25}
$\bm{\hat{x}}$ & 49.0 & 130.0 & 265.98 & 171.01 & 0.6 & atypical angina & normal & no & false & male & upsloping & normal & 0 \\
\rowcolor{gray!10} 
\multicolumn{14}{l}{\cellcolor[HTML]{EFEFEF}\textbf{Part A}: validity, proximity, coherence} \\

(a) & 48.82 & 139.28 & 328.09 & 153.98 & 1.05 & - & - & - & - & - & - & - & - \\
\rowcolor{gray!10} 
\multicolumn{14}{l}{\cellcolor[HTML]{EFEFEF}\textbf{Part B}: validity, proximity, coherence, sparsity} \\

(a) & - & - & 407.24 & - & - & - & - & - & - & - & - & - & - \\
\rowcolor{gray!10} 
\multicolumn{14}{l}{\cellcolor[HTML]{EFEFEF}\textbf{Part C}: validity, proximity, coherence, sparsity, diversity} \\

(a) & - & - & 407.24 & - & - & - & - & - & - & - & - & - & - \\

(b) & - & - & 393.92 & 175.14 & - & - & - & - & - & - & - & - & - \\

(c) & - & - & 404.04 & - & 0.47 & - & - & - & - & - & - & - & - \\
\rowcolor{gray!10} 
\multicolumn{14}{l}{\cellcolor[HTML]{EFEFEF}\textbf{Part D}: validity, proximity, coherence, sparsity, diversity, actionability} \\

(a) & - & - & 407.24 & - & - & - & - & - & - & - & - & - & - \\

(b) & - & - & 393.92 & 175.14 & - & - & - & - & - & - & - & - & - \\

(c) & - & - & - & 124.37 & - & - & - & - & - & - & - & - & - \\
\rowcolor{gray!10} 
\multicolumn{14}{l}{\cellcolor[HTML]{EFEFEF}\textbf{Part E}: validity, proximity, coherence, sparsity, diversity, actionability, data manifold closeness} \\

(a) & - & 111.77 & 253.81 & 152.7 & 0.0 & nonanginal pain & - & - & - & - & - & - & - \\

(b) & - & 137.0 & 258.5 & 147.01 & 1.55 & asymptomatic & left ventricular hypertrophy & - & - & - & flat & reversible defect & - \\

(c) & - & 140.61 & 274.7 & 128.61 & 0.49 & asymptomatic & left ventricular hypertrophy & yes & - & - & - & reversible defect & - \\ \bottomrule

\multicolumn{14}{l}{See Table \ref{tab:description-heart}  for a description of each feature} \\[-2mm]
\multicolumn{14}{l}{The dash (--) represents no change in a feature with respect to the factual instance.} \\[-2mm]

\end{tabular}
}

\vspace{0.4cm}
% \normalsize
% \begin{subtable}

        \centering
        % \caption{Evaluation$^*$ of counterfactuals generated for a single factual instance, with constraints added gradually.}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{lcccccc}
        % \begin{tabular}{p{1.2cm}p{2cm}p{2.2cm}p{2cm}p{2cm}p{2cm}p{2.5cm}p{2.5cm}}
        
        \multicolumn{7}{l}{\normalsize{(b) Evaluation$^*$ of counterfactuals generated for a single factual instance, with constraints added gradually.}} \\
% \multicolumn{7}{l}{constraint presented in Section~\ref{sec:generate}} \\

        \toprule
        
        {} &  \small \textbf{categorical} &  \small\textbf{continuous} &  \small\textbf{sparsity}($\uparrow_0^1$) &  \small\textbf{categorical} &  \small\textbf{continuous} &  \small\textbf{sparsity-based} \\ [-2mm]
        
        {} &  \small\textbf{proximity}($\uparrow_0^1$) &  \small\textbf{proximity}($\uparrow_-^0$) &   & \small \textbf{diversity}($\uparrow_0^1$) &  \small\textbf{diversity}($\uparrow_0^+$) &  \small\textbf{diversity}($\uparrow_0^1$) \\
        

        % \multicolumn{7}{l}{(b) Evaluation$^*$ of counterfactuals generated for a single factual instance, with constraints added gradually.}\\
        % \toprule
        % {} &  \textbf{categorical proximity}($\uparrow_0^1$) &  \textbf{continuous proximity}($\uparrow_-^0$) &  \textbf{sparsity}($\uparrow_0^1$) &  \textbf{categorical diversity}($\uparrow_0^1$) &  \textbf{continuous diversity}($\uparrow_0^+$) &  \textbf{sparsity-based diversity}($\uparrow_0^1$) \\
        \midrule
        \rowcolor{gray!10}
        \small Part A  & \small 1.00 & \small -89.05 & \small 0.62 & - & - & - \\
        \small Part B  & \small 1.00 &\small  -141.26 & \small 0.92 & - & - & - \\
        \rowcolor{gray!10}
        \small Part C  & \small 1.00 & \small -137.17 & \small 0.87 & \small 0.00 & \small 11.72 & \small 0.18 \\ 
        \small Part D  & \small  1.00 & \small -106.66 & \small 0.90 & \small 0.00 & \small 128.02 & \small 0.15 \\
        \rowcolor{gray!10} 
        \small Part E  & \small 0.62 & \small -50.19 & \small 0.46 & \small 0.42 & \small 50.25 & \small 0.56\\ \bottomrule
        
\multicolumn{7}{l}{\footnotesize \textbf{Part A:} validity, proximity, coherence; \textbf{Part B:} validity, proximity, coherence, sparsity; \textbf{Part C:} validity, proximity, coherence, } \\[-3mm]

\multicolumn{7}{l}{\footnotesize sparsity, diversity; \textbf{Part D:} validity, proximity, coherence, sparsity, diversity, actionability; \textbf{Part E:} validity, proximity, coherence, } \\[-3mm]

\multicolumn{7}{l}{\footnotesize sparsity, diversity, actionability, data manifold closeness; \textbf{Part F:} validity, proximity, coherence, sparsity, diversity, actionability.} \\ [-3mm]

\multicolumn{7}{l}{\footnotesize data manifold closeness, causality} \\ [-3mm]
        \multicolumn{7}{l}{\footnotesize \textbf{$^*$validity ($\uparrow_0^1$):} 1.00 in all cases}\\
        %\bottomrule
      \end{tabular}}
    %   \end{tabular}
       \label{tab:heart_demo}
% \end{subtable}

\end{table}

==> CE-OCL arXiv 2/tables/table_demonstration.tex <==
\renewcommand{\baselinestretch}{1.2} 

\begin{table}[ht]
\caption{\protect \texttt{CE-OCL} demo on the Statlog (German Credit Data) Data Set \citep[][]{Dua:2019}.}
% \begin{subtable}[h]{\textwidth}
% \begin{subtable}
\centering
% \caption{Counterfactual explanations generated for enriching the optimization model step by step with the constraint presented in Section~\ref{sec:generate}}.
% \subtabcap{Counterfactual explanations generated for enriching the optimization model step by step with the constraint presented in Section~\ref{sec:generate}}.
% \vspace{0.1cm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{1cm}p{1cm}p{1.4cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1.4cm}p{1cm}p{1cm}p{1cm}}

\multicolumn{12}{l}{(a) Counterfactual explanations generated for enriching the optimization model step by step with the} \\
\multicolumn{12}{l}{constraint presented in Section~\ref{sec:generate}} \\

\toprule

{} &     F1 &       F2 &    F3 &     F4 &   F8$^*$ &     F10 &   F12 &        F14 &   F16 & F18$^*$ & F20$^*$ \\
\midrule
\rowcolor{gray!25} $\hat{\bm{x}}$ &   24.0 &  1371.26 &   4.0 &   25.0 &  A &   1$\leq$X$<$4 &  rent &       none &  none &   A &   A \\


%\hline
\rowcolor{gray!10}\multicolumn{12}{l}{\textbf{Part A}: validity, proximity, coherence} \\
%\hline

(a)     &  15.02 &	-333.52	& 3.86 &	27.04 &  -- &       -- &     -- &          -- &     -- &   -- &   -- \\


%\hline
\rowcolor{gray!10}\multicolumn{12}{l}{\textbf{Part B}: validity, proximity, coherence, sparsity} \\
%\hline

(a)     &   7.12 & -- &     -- &  -- &  -- &       -- &     -- &          -- &     -- &   -- &   -- \\

%\hline
\rowcolor{gray!10}\multicolumn{12}{l}{\textbf{Part C}: validity, proximity, coherence, sparsity, diversity} \\
%\hline

(a)     &   7.12 &     -- &     -- &  -- &  -- &       -- &     -- &          -- &     -- &   -- &   -- \\
(b)     &      -- & -2873.47 &     -- &      30.06 &  -- &       -- &     -- &          -- &     -- &   -- &   -- \\
(c)     &      -- &        -- &     1.96 &      26.63 & -- &       -- &     -- &          -- &     -- &   -- &   -- \\

%\hline
\rowcolor{gray!10}\multicolumn{12}{l}{\textbf{Part D}: validity, proximity, coherence, sparsity, diversity, actionability} \\
%\hline

(a)     &   7.12 &  -- &     -- &  -- &  -- &       -- &     -- &  -- &     -- &   -- &   -- \\
(b) & -- &  -- &  1.96 &  26.63 &  -- &  -- &     -- &  -- &     -- &   -- &   -- \\
(c) &  -- &  -- &  -- &  75.52 &   -- &  -- &     -- &  -- &  -- &   -- &   -- \\

%\hline
\rowcolor{gray!10}\multicolumn{12}{l}{\textbf{Part E}: validity, proximity, coherence, sparsity, diversity, actionability, data manifold closeness} \\
%\hline

(a)     &   22.0 &  1283.52 &     -- &      -- &  B &   4$\leq$X$<$7 &     -- &          -- &     -- &   B &   -- \\
(b)     &      10 &  1363.43 &     2.0 &   64.0 &  B &       -- &     own &          -- &   yes &   C &   B \\
(c)     &   12.0 &  1893.04 &     -- &   29.0 &  -- &       -- &   own &  guarantor &   yes &   B &   B \\


%\hline
\rowcolor{gray!10}
\multicolumn{12}{l}{\textbf{Part F}: validity, proximity, coherence, sparsity, diversity, actionability, data manifold closeness, causality} \\
%\hline
(a)     &      -- &        -- &     -- &      --  &  B &  4<=X<7 &     -- &          -- &     -- &   B &   -- \\
(b)     &   22.0 &   990.51 &     -- &      -- &  B &   4<=X<7 &     -- &          -- &     -- &   B &   -- \\
(c)     &  26.83 &  1910.28 &     -- &      -- &  B &  4<=X<7 &     -- &          -- &     -- &   B &   -- \\

\bottomrule

\multicolumn{12}{l}{\footnotesize F1--F20 represent the 20 features of the dataset. See Table \ref{tab:description} in Appendix \ref{app:case study} for a description.} \\[-2mm]
\multicolumn{12}{l}{\footnotesize The dash (--) represents no change in a feature with respect to the factual instance.} \\[-2mm]
\multicolumn{12}{l}{\footnotesize\textbf{F5, F6, F7, F9, F11, F13, F15, F17, F19:} None of the counterfactual explanations proposed a change in these variables. For space }\\[-2mm]
\multicolumn{12}{l}{\footnotesize reasons they are not displayed here.} \\[-2mm]
\multicolumn{12}{l}{\footnotesize $^*$ \textbf{F8:} A: $$<$$0, B: no checking; \textbf{F18:} A: real estate, B: life insurance, C: car ; \textbf{F20:} A: no known savings, B: $$<$$100} \\
\end{tabular}}
% \label{tab:display_demo}
% \end{subtable}
% \hfill
% \begin{subtable}[h]{\textwidth}

\vspace{0.4cm}
% \normalsize
% \begin{subtable}

        \centering
        % \caption{Evaluation$^*$ of counterfactuals generated for a single factual instance, with constraints added gradually.}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{lcccccc}
        % \begin{tabular}{p{1.2cm}p{2cm}p{2.2cm}p{2cm}p{2cm}p{2cm}p{2.5cm}p{2.5cm}}
        
        \multicolumn{7}{l}{\normalsize{(b) Evaluation$^*$ of counterfactuals generated for a single factual instance, with constraints added gradually.}} \\
% \multicolumn{7}{l}{constraint presented in Section~\ref{sec:generate}} \\

        \toprule
        
        {} &  \small \textbf{categorical} &  \small\textbf{continuous} &  \small\textbf{sparsity}($\uparrow_0^1$) &  \small\textbf{categorical} &  \small\textbf{continuous} &  \small\textbf{sparsity-based} \\ [-2mm]
        
        {} &  \small\textbf{proximity}($\uparrow_0^1$) &  \small\textbf{proximity}($\uparrow_-^0$) &   & \small \textbf{diversity}($\uparrow_0^1$) &  \small\textbf{diversity}($\uparrow_0^+$) &  \small\textbf{diversity}($\uparrow_0^1$) \\
        
        \midrule
\small Part A & \small               1.00 & \small  -1715.94 &   \small   0.8 &        -- &         -- &                -- \\
\rowcolor{gray!10} \small Part B &              \small  1.00 &    \small  -16.88 &    \small   0.95 &        -- &         -- &                -- \\
\small Part C &             \small   1.00 &  \small  -1423.45 &    \small   0.92 &    \small    0.00 &    \small  2845.81 &         \small       0.15 \\
\rowcolor{gray!10}\small Part D &            \small    1.00 & \small     -23.69 &  \small     0.93 &     \small   0.00 &   \small     46.29 &   \small             0.12 \\
\small Part E &        \small        0.67 &   \small  -230.12 &    \small   0.63 &     \small   0.36 &     \small  441.68 & 0.42 \\
\rowcolor{gray!10}\small Part F &       \small         0.77 & \small    -308.20 &   \small    0.78 &      \small  0.00 &   \small    616.40 &        \small        0.10 \\

%Part F &         1 &      0.77 &    -157.50 &      0.78 &       0.00 &      255.17 &               0.08 \\
        \bottomrule
\multicolumn{7}{l}{\footnotesize \textbf{Part A:} validity, proximity, coherence; \textbf{Part B:} validity, proximity, coherence, sparsity; \textbf{Part C:} validity, proximity, coherence, } \\[-2mm]
\multicolumn{7}{l}{\footnotesize sparsity, diversity; \textbf{Part D:} validity, proximity, coherence, sparsity, diversity, actionability; \textbf{Part E:} validity, proximity, coherence, } \\[-2mm]
\multicolumn{7}{l}{\footnotesize sparsity, diversity, actionability, data manifold closeness; \textbf{Part F:} validity, proximity, coherence, sparsity, diversity, actionability.} \\ [-2mm]
\multicolumn{7}{l}{\footnotesize data manifold closeness, causality} \\ [-2mm]
\multicolumn{7}{l}{\footnotesize \textbf{$^*$validity ($\uparrow_0^1$):} 1.00 in all cases } \\ 
        % \multicolumn{7}{l}{\footnotesize \textbf{$^*$validity ($\uparrow_0^1$):} 1.00 in all cases}
        %\bottomrule
      \end{tabular}}
    %   \end{tabular}
       \label{tab:credit_demo}
% \end{subtable}

\end{table}


==> CE-OCL arXiv 2/tables/table_description.tex <==
\renewcommand{\baselinestretch}{1.5} 

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\caption{Information on Statlog (German Credit Data) Data Set \protect \citep[][]{Dua:2019}}
\label{tab:description}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Label} & \textbf{Variable name} & \textbf{Description} & \textbf{Domain$*$} & \textbf{Constraint} \\ \midrule
F1 & duration & Duration in months & real & $\geq 0$ \\
\rowcolor{gray!10}F2 & credit\_amount & Credit amount & real & $\geq 0$ \\
F3 & instalment\_commitment & Installment rate in percentage of disposable income & real & $\geq 0$ \\
\rowcolor{gray!10}F4 & age & Age in years & real & $x_{age} \geq \hat{\vx}_{age}$ \\
F5 & residence\_since & Present residence since X years & integer  & $x_{residence\_since} \geq \hat{\vx}_{residence\_since}$ \\
\rowcolor{gray!10}F6 & existing\_credits & Number of existing credits at this bank & integer & $\geq 0$ \\
F7 & num\_dependents & Number of people being liable to provide maintenance for & integer & $\geq 0$ \\
\rowcolor{gray!10}F8 & checking\_status & Status of existing checking account, in Deutsche Mark & binary & -- \\
F9 & credit\_history & Credit history (credits taken, paid back duly, delays, critical accounts) & binary & -- \\
\rowcolor{gray!10}F10 & employment & Present employment, in number of years. & binary & conditionally immutable \\
F11 & foreign\_worker & Foreign worker (yes,no) & binary & immutable \\
\rowcolor{gray!10}F12 & housing & Housing (rent, own,...) & binary & -- \\
F13 & job & Job & binary & -- \\
\rowcolor{gray!10}F14 & other\_parties & Other debtors / guarantors & binary & -- \\
F15 & other\_payment\_plans & Other installment plans (banks, stores) & binary & -- \\
\rowcolor{gray!10}F16 & own\_telephone & Telephone (yes,no) & binary & -- \\
F17 & personal\_status & Personal status (married, single,...) and sex & binary & \begin{tabular}[c]{@{}l@{}}immutable\end{tabular} \\
\rowcolor{gray!10}F18 & property\_magnitude & Property (e.g. real estate) & binary & -- \\
F19 & purpose & Purpose of the credit (car, television,...) & binary & \begin{tabular}[c]{@{}l@{}}immutable \end{tabular} \\
\rowcolor{gray!10}F20 & saving\_status & Status of savings account/bonds, in Deutsche Mark. & binary & -- \\ \bottomrule
\multicolumn{5}{l}{\footnotesize $^*$ All categorical are one-hot encoded and therefore considered binary.}
\end{tabular}}
\end{table}

==> CE-OCL arXiv 2/tables/table_heart_description.tex <==
\renewcommand{\baselinestretch}{1.1} 

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\centering
\caption{Information on Statlog (Heart) Data Set \protect \citep[][]{Dua:2019}}
\label{tab:description-heart}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{llll}
\toprule
\textbf{Variable name} & \textbf{Description} & \textbf{Domain$*$} & \textbf{Constraint} \\ \midrule
\rowcolor{gray!10}age & Patient age in years & real & immutable \\
sex & Gender & binary & immutable \\
\rowcolor{gray!10}chp & Chest pain type & binary & - \\
bp & Resting blood pressure & real & $\geq 0$ \\
\rowcolor{gray!10}sch & Serum cholesterol & real & $\geq 0$ \\
fbs & Fasting blood sugar \textgreater 120 mg/dL & binary & - \\
\rowcolor{gray!10}ecg & Resting electrocardiographic result & binary & - \\
mhrt & Maximum heart rate & real & $\geq 0$ \\
\rowcolor{gray!10}exian & Exercise induced angina & binary & - \\
opk & Old peak & real & $\geq 0$ \\
\rowcolor{gray!10}slope & Slope of peak exercise ST segment & binary & - \\
vessel & Number of major  vessels & binary & - \\
\rowcolor{gray!10}thal & Defect type & binary & - \\ \bottomrule
\multicolumn{4}{l}{\footnotesize $^*$ All categorical are one-hot encoded and therefore considered binary.}
\end{tabular}}
\end{table}

==> CE-OCL arXiv 2/tables/table_overview.tex <==
\renewcommand{\baselinestretch}{1.1} 

\begin{table}[ht]
\caption{State-of-the-art methods to generate CEs}
\label{tab:overview}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule

& \textbf{Proximity} & \textbf{Sparsity} & \textbf{Coherence} & \textbf{Actionability} & \textbf{Data Manifold Closeness} & \textbf{Causality} & \textbf{Diversity} \\ \midrule
\rowcolor{gray!10} \citet{Laugel2017} & \CIRCLE & \CIRCLE & \CIRCLE & -- & -- & -- & -- \\ 
\citet{Russell.2019}  & \CIRCLE & \LEFTcircle & \CIRCLE & -- & -- & -- & \CIRCLE \\
\rowcolor{gray!10}\citet{Ustun.2019} &  \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & -- & -- & -- \\
\citet{Kanamori.2020} & \CIRCLE & -- & \CIRCLE & -- & \CIRCLE & -- & -- \\
\rowcolor{gray!10}\citet{Mahajan.2019} & \CIRCLE & -- & \CIRCLE & \LEFTcircle & \CIRCLE & \CIRCLE & -- \\
%\citet{Sharma2020} & \CIRCLE & -- & \CIRCLE & -- & -- & -- & \CIRCLE \\
\citet{Karimi.2020} & \CIRCLE & -- & \CIRCLE & -- & -- & \CIRCLE & -- \\
\rowcolor{gray!10}\citet{Kanamori.2020jn} & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & -- & \CIRCLE & \CIRCLE \\
%MACE \citet{Karimi.2019fy} & model-agnostic  &  &  &  &  &  &  &  \\
\citet{Mothilal.2020} & \CIRCLE & \LEFTcircle & \CIRCLE & \CIRCLE & -- & \LEFTcircle &\CIRCLE \\
\rowcolor{gray!10}\citet{Karimi.2019fy} & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & -- & -- &\CIRCLE \\
\citet{Poyiadzi2020} & \CIRCLE & -- & \CIRCLE & \CIRCLE & \CIRCLE & -- & -- \\
\rowcolor{gray!10}\texttt{CE-OCL} & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE \\ \bottomrule
\multicolumn{8}{l}{\footnotesize \CIRCLE: addressed; \LEFTcircle: partially addressed; --: absent}

\end{tabular}}
\end{table}


